DebUnc: Improving Large Language Model Agent Communication With Uncertainty Metrics

Multi-agent debates have been introduced to improve the accuracy of Large Language Models (LLMs) by having multiple agents discuss solutions to a problem over several rounds of debate. However, models often generate incorrect yet confident-sounding responses, which can mislead others. This issue arises partly because agents do not consider how confident their peers are. To address this, we propose DebUnc, a debate framework that uses uncertainty metrics to assess agent confidence. Confidence is then conveyed through a modified attention mechanism that adjusts token weights, or through textual prompts. Evaluations across benchmarks show that attention-based methods are particularly effective and that performance continues to improve as uncertainty estimation becomes more reliable. The code is available at https://github.com/lukeyoffe/debunc.

==> tables/llama.tex <==

\begin{table*}[h]
    \centering
    \begin{tabular}{llccccc}
        \toprule
        \textbf{Metric} & \textbf{Method}  & \textbf{MMLU-0} & \textbf{GSM8k} & \textbf{TruthfulQA} & \textbf{Arithmetic} & \textbf{Average} \\
        \midrule
        N/A               & Standard Debate   & 0.654           & 0.812          & 0.518               & 0.520          & 0.634 \sfns +0.0\%
 \\
        \midrule                      
        Entropy           & Prompt            & 0.614           & \textbf{0.840} & 0.540               & 0.528          & 0.636 \textcolor{green}{\sfns +0.4\%}
 \\
                          & Attention-Others  & 0.638           & 0.810          & \textbf{0.562}      & 0.526          & \textbf{0.639} \textcolor{green}{\sfns +0.9\%}
 \\
                          & Attention-All     & \textbf{0.658}  & 0.808          & 0.556               & \textbf{0.530} & 0.638 \textcolor{green}{\sfns +0.4\%}
 \\
        \midrule             
        Oracle*           & Prompt            & 0.668           & 0.872          & 0.584               & 0.546          & 0.668 \textcolor{green}{\sfns +5.5\%}
 \\
                          & Attention-Others  & \textbf{0.784}  & 0.898          & 0.674               & \textbf{0.556} & \textbf{0.728} \textcolor{green}{\sfns +14.9\%}
 \\
                          & Attention-All     & 0.754           & \textbf{0.900} & \textbf{0.682}      & \textbf{0.556} & \textbf{0.728} \textcolor{green}{\sfns +15.0\%}  \\
        \bottomrule
    \end{tabular}
    \caption{Accuracy comparison across various benchmarks using different uncertainty metrics (* the oracle metric simulates a perfect metric) and communication methods with Llama-3-8B. Zero-shot prompting was used for all benchmarks. The `Average' column shows the average performance over all benchmarks and the \textcolor{green}{\% increase} over the standard debate.}
    \label{table:llama}
\end{table*}

==> tables/mistral.tex <==
\begin{table*}
\centering
\begin{tabular}{llcccccc}
\toprule
\textbf{Metric} & \textbf{Method} & \textbf{MMLU-0} & \textbf{MMLU-5} & \textbf{GSM8k} & \textbf{Arith.} & \textbf{Truth.} & \textbf{Average}\\
\midrule
     --- & Standard Debate & 0.520 & 0.544 & 0.512 & 0.478 & 0.604 & 0.532 \sfns +0.0\% \\
\midrule
% \multirow[t]{3}{*}{Prompt} 
 Entropy & Prompt & 0.522 & 0.546 & \textbf{0.536} & 0.482 & 0.602 & 0.538 \textcolor{green}{\sfns +1.1\%} \\
 & Attn-Others  & \textbf{0.540} & 0.566 & 0.488 & \textbf{0.518} & \textbf{0.608} & 0.544 \textcolor{green}{\sfns +2.3\%} \\
 & Attn-All  & 0.526 & \textbf{0.570} & \textbf{0.536} & \textbf{0.518} & 0.604 & \textbf{0.551} \textcolor{green}{\sfns +3.6\%} \\
\midrule
% \multirow[t]{3}{*}{Attention-Others}
 TokenSAR & Prompt & \textbf{0.538} & 0.548 & 0.504 & 0.464 & 0.616 & 0.534 \textcolor{green}{\sfns +0.4\%} \\
 & Attn-Others  & 0.526 & \textbf{0.560} & 0.496 & \textbf{0.500} & \textbf{0.626} & 0.542 \textcolor{green}{\sfns +1.9\%} \\
 & Attn-All  & 0.532 & 0.552 & \textbf{0.528} & \textbf{0.500} & 0.610 & \textbf{0.544} \textcolor{green}{\sfns +2.3\%} \\
\midrule
% \multirow[t]{3}{*}{Attention-All} 
 Oracle* & Prompt & 0.562 & 0.560 & 0.548 & 0.542 & 0.626 & 0.568 \textcolor{green}{\sfns +6.8\%} \\
 & Attn-Others  & 0.606 & 0.666 & 0.640 & 0.654 & 0.630 & 0.639 \textcolor{green}{\sfns +20.1\%} \\
 & Attn-All  & \textbf{0.618} & \textbf{0.684} & \textbf{0.656} & \textbf{0.732} & \textbf{0.648} & \textbf{0.668} \textcolor{green}{\sfns +25.6\%} \\
\bottomrule
\end{tabular}
\caption{Accuracy comparison across various benchmarks using different uncertainty metrics (* the oracle metric simulates a perfect metric) and communication methods with Mistral-7B. `MMLU-0' and `MMLU-5' represent 0 and 5-shot performance on MMLU respectively. The other benchmarks used zero-shot prompting. The `Average' column shows the average performance over all benchmarks and the \textcolor{green}{\% increase} over the standard debate.}
\label{table:comparison}
\end{table*}
